Cluster-based network modeling -- automated robust modeling of complex dynamical systems

We propose a universal method for data-driven modeling of complex nonlinear dynamics from time-resolved snapshot data without prior knowledge. Complex nonlinear dynamics govern many fields of science and engineering. Data-driven dynamic modeling often assumes a low-dimensional subspace or manifold for the state. We liberate ourselves from this assumption by proposing cluster-based network modeling (CNM) bridging machine learning, network science, and statistical physics. CNM only assumes smoothness of the dynamics in the state space, robustly describes short- and long-term behavior and is fully automatable as it does not rely on application-specific knowledge. CNM is demonstrated for the Lorenz attractor, ECG heartbeat signals, Kolmogorov flow, and a high-dimensional actuated turbulent boundary layer. Even the notoriously difficult modeling benchmark of rare events in the Kolmogorov flow is solved. This automatable universal data-driven representation of complex nonlinear dynamics complements and expands network connectivity science and promises new fast-track avenues to understand, estimate, predict and control complex systems in all scientific fields.

==> build <==
#!/bin/bash

pdflatex --shell-escape $1 &&
bibtex $1 &&
pdflatex --shell-escape $1 &&
pdflatex --shell-escape $1 &&

# Extract the citations into 'citations'
echo "Extract the citations"
cat Main.aux | grep "\\\\citation" | sed 's/\\citation{\(.*\)}/\1/g' | uniq > citations

# Clean the folder
./clean



==> clean <==
#!/bin/bash

function nettoie() {
  while [ -n "$1" ] ; do
    nom=$1
    rm $nom/*.toc 2>/dev/null
    rm $nom/*.mtc* 2>/dev/null
    rm $nom/*.dvi 2>/dev/null
    rm $nom/*.dvi 2>/dev/null
    rm $nom/*.out 2>/dev/null
    rm $nom/*.lof 2>/dev/null
    rm $nom/*.lot 2>/dev/null
    rm $nom/*.aux 2>/dev/null
    rm $nom/*.idx 2>/dev/null
    rm $nom/*.ilg 2>/dev/null
    rm $nom/*.ind 2>/dev/null
    rm $nom/*.log 2>/dev/null
    rm $nom/*.*# 2>/dev/null
    rm $nom/*.tex~ 2>/dev/null
    #rm $nom/*.bbl 2>/dev/null
    rm $nom/*.brf 2>/dev/null
    rm $nom/*.bmt 2>/dev/null
    rm $nom/*.blg 2>/dev/null
    rm $nom/*~ 2>/dev/null
    rm $nom/.*~ 2>/dev/null
    rm core 2>/dev/null
    echo -e '\E[34m' "Rep $nom :" '\E[0m' `ls $nom`
    shift
  done
}

nom=`pwd`
nettoie $nom

for i in `ls` ; do
  if [ -d "$i" ] ; then nettoie $i ; fi
done

